Exact and Heuristic Approaches for the Stochastic N-k Interdiction in Power Grids

The article introduces the stochastic N-k interdiction problem for power grid operations and planning that aims to identify a subset of k components (out of N components) that maximizes the expected damage, measured in terms of load shed. Uncertainty is modeled through a fixed set of outage scenarios, where each scenario represents a subset of components removed from the grid. We formulate the stochastic N-k interdiction problem as a bi-level optimization problem and propose two algorithmic solutions. The first approach reformulates the bi-level stochastic optimization problem to a single level, mixed-integer linear program (MILP) by dualizing the inner problem and solving the resulting problem directly using a MILP solver to global optimality. The second is a heuristic cutting-plane approach, which is exact under certain assumptions. We compare these approaches in terms of computation time and solution quality using the IEEE-Reliability Test System and present avenues for future research.

==> scratch.tex <==
\section{Formulation}
\begin{flalign}
& (\mathcal F_1) \quad z =  \max \, \sum_{s \in \mathcal S} \bm{Pr}_s \eta_s(\bm x,\bm y) \text{ subject to:} & \label{eq:obj_outer} \\
& \sum_{(i,j) \in \mathcal E} x_{ij} + \sum_{i \in \mathcal N} y_i \leqslant \bm k \text{ and } (\bm x, \bm y) \in \mathbb B^n & \label{eq:x}
\end{flalign}
where
\begin{flalign}
& (\text{PLS}_s(\bm x, \bm y)) \quad \eta_s(\bm x, \bm y) = \min \, \sum_{i \in {\mathcal N}} \bm p^d_i \ell_i^s \text{ subject to:}& \label{eq:obj_inner} \\
& p_i^{gs} - (1-\ell_i^s)\bm p_i^d = \sum_{(i,j) \in \mathcal E \bigcup \mathcal E^r} p_{ij}^s \quad \forall i\in \mathcal N, & \label{eq:kcl} \\
& p^{gs}_i \geqslant (1-y_i\xi_i^s)\, \bm p^{gl}_i  \quad \forall i \in \mathcal N, &\label{eq:pg_1} \\
& p^{gs}_i \leqslant (1-y_i\xi_i^s)\, \bm p^{gu}_i \quad \forall i\in \mathcal N, & \label{eq:pg_2} \\
& p_{ij}^s  \geqslant -\bm t_{ij} (1 - x_{ij}{\xi}_{ij}^s) \quad \forall (i,j) \in \mathcal E, & \label{eq:thermal_1} \\
& p_{ij}^s  \leqslant \bm t_{ij} (1 - x_{ij}{\xi}_{ij}^s) \quad \forall (i,j) \in \mathcal E, & \label{eq:thermal_2} \\
& p_{ij}^s + \bm b_{ij} (\theta^s_i - \theta^s_j) \geqslant -M x_{ij} \xi_{ij}^s  \quad \forall (i,j) \in \mathcal E, & \label{eq:pij_1} & \\
& p_{ij}^s + \bm b_{ij} (\theta^s_i - \theta^s_j) \leqslant M x_{ij} \xi_{ij}^s  \quad \forall (i,j) \in \mathcal E, \label{eq:pij_2} & \\
& \theta^s_i - \theta^s_j \geqslant -\bm \theta_{ij} (1-x_{ij}\xi_{ij}^s) - \bm \theta^M x_{ij}\xi_{ij}^s \quad \forall (i,j) \in \mathcal E, \label{eq:thetaij_1} & \\
& \theta^s_i - \theta^s_j \leqslant \bm \theta_{ij} (1-x_{ij}\xi_{ij}^s) + \bm \theta^M x_{ij}\xi_{ij}^s \quad \forall (i,j) \in \mathcal E, \label{eq:thetaij_2} & \\
&\ell_i^s \leqslant 1 \quad \forall i \in \mathcal N, & \label{eq:loadshed_2} \\
&\ell_i^s \geqslant 0 \quad \forall i \in \mathcal N. & \label{eq:loadshed_1}
\end{flalign}


Let $\alpha_i^s, \beta_i^{s+}, \beta_i^{s-}, \gamma_{ij}^{s+}, \gamma_{ij}^{s-}, \delta_{ij}^{s+}, \delta_{ij}^{s-},\eta_{ij}^{s+}, \eta_{ij}^{s-},\text{ and }\omega_i^s$ denote the dual variables corresponding to \eqref{eq:kcl}, \eqref{eq:pg_1}, \eqref{eq:pg_2}, \eqref{eq:thermal_1}, \eqref{eq:thermal_2}, \eqref{eq:pij_1}, \eqref{eq:pij_2}, \eqref{eq:thetaij_1}, \eqref{eq:thetaij_2}, and \eqref{eq:loadshed_2}, respectively. Then the dual of the inner problem PLS$_s(\bm x, \bm y)$ is as follows: 
\begin{flalign}
& (\text{DLS}_s(\bm x, \bm y)) \quad \Delta_s(\bm x, \bm y) = \max \sum_{i \in \mathcal N} \left\{ (1-y_i \xi_i^s) \left[ \bm p_i^{gl} \beta_i^{s+} -  \right. \right. & \notag \\
& \quad \left. \left. \bm p_i^{gu} \beta_i^{s-} \right] - \omega_i^s - \bm p_i^d \alpha_i^s \right\} - \sum_{(i,j) \in \mathcal E} \left\{ Mx_{ij}\xi_{ij}^s \left[ \delta_{ij}^{s+} + \delta_{ij}^{s-} \right] \right. & \notag  \\
& \quad + \left( \bm \theta_{ij} (1-x_{ij}\xi_{ij}^s) + \bm \theta^M x_{ij}\xi_{ij}^s\right) \left[ \eta_{ij}^{s+} + \eta_{ij}^{s-}\right] & \notag \\
& \quad \left. + \,\bm t_{ij} (1 - x_{ij}{\xi}_{ij}^s) \left[ \gamma_{ij}^{s+} + \gamma_{ij}^{s-} \right] \right\} \text{ subject to: } & \label{eq:obj_dual} \\
& \alpha_i^s - \alpha_j^s + \gamma_{ij}^{s+} - \gamma_{ij}^{s-} + \delta_{ij}^{s+} - \delta_{ij}^{s-} = 0 \quad \forall (i,j) \in \mathcal E, & \label{eq:pij_d} \\
& \sum_{(i,j) \in \mathcal E \cup \mathcal E^r} \left\{ b_{ij}\left[ \delta_{ij}^{s+} - \delta_{ij}^{s-} \right] + \eta_{ij}^{s+} - \eta_{ij}^{s-} \right\} = 0 \quad \forall i \in \mathcal N, & \label{eq:theta_d} \\
& -\alpha_i^s + \beta_i^{s+} - \beta_i^{s-} = 0 \quad \forall i \in \mathcal N, & \label{eq:pg_d} \\
& -\bm p_i^d \alpha_i^s - \omega_i^s \leqslant \bm p_i^d \quad \forall i \in \mathcal N, & \label{eq:l_d} \\
& \beta_i^{s+}, \beta_i^{s-}, \omega_i^s \geqslant 0 \quad \forall i \in \mathcal N, & \label{eq:nn_1} \\
& \gamma_{ij}^{s+}, \gamma_{ij}^{s-}, \delta_{ij}^{s+}, \delta_{ij}^{s-} \geqslant 0 \quad \forall (i,j) \in \mathcal E. & \label{eq:nn_2}
\end{flalign}
When $\bm p_i^{gl} = 0$ for every $i\in \mathcal N$, the inner primal problem, PLS$_s(\bm x, \bm y)$, is never empty for any interdiction plan $(\bm x, \bm y)$ and any scenario $s$ \emph{i.e.}, $\bm 0 \in \text{PLS}_s(\bm x, \bm y)$. We also remark that the objective value of the primal inner problem PLS$_s(\bm x, \bm y)$ is bounded for all $(\bm x, \bm y) \in \mathbb{B}^n$. Since, PLS$_s(\bm x, \bm y)$ is nonempty and bounded for all $(\bm x, \bm y)$ and $s$, the strong duality theorem of linear programming indicates that for any interdiction $(\hat{\bm x}, \hat{\bm y})$ and scenario $s$, if there exists primal and dual solution such that 
\begin{flalign}
& \sum_{i \in \mathcal N} \bm p_i^d \ell_i^{s*} = \sum_{i \in \mathcal N} \left\{ (1-y_i \xi_i^s) \left[ \bm p_i^{gl} \beta_i^{s+*} -  \bm p_i^{gu} \beta_i^{s-*}  \right]  - \omega_i^{s*} \right. & \notag \\
& \qquad \left. - \bm p_i^d \alpha_i^{s*} \right\} - \sum_{(i,j) \in \mathcal E} \left\{ Mx_{ij}\xi_{ij}^{s} \left[ \delta_{ij}^{s+*} + \delta_{ij}^{s-*} \right] \right.  & \notag  \\
& \qquad  +  \left( \bm \theta_{ij} (1-x_{ij}\xi_{ij}^{s*}) + \bm \theta^M x_{ij}\xi_{ij}^{s*}\right) \left[ \eta_{ij}^{s+*} + \eta_{ij}^{s-*}\right] & \notag \\
& \qquad \left. +\, \bm t_{ij} (1 - x_{ij}{\xi}_{ij}^{s}) \left[ \gamma_{ij}^{s+*} + \gamma_{ij}^{s-*} \right] \right\} & \label{eq:sd}
\end{flalign}
then, $\sum_{i \in \mathcal N} \bm p_i^d \ell_i^{s*} = \eta_s(\bm x, \bm y)$. The above result yields a single level formulation for the problem. We will refer to the resulting formulation as $\mathcal F_2$
\begin{flalign}
& (\mathcal F_2) \quad z =  \max \, \sum_{s \in \mathcal S} \bm{Pr}_s \left( \sum_{i \in \mathcal N} \bm p_i^d \ell_i^{s} \right)\text{ subject to:} & \label{eq:obj_outer_n} \\
& \sum_{i \in \mathcal N} \bm p_i^d \ell_i^{s} = \sum_{i \in \mathcal N} \left\{ (1-y_i \xi_i^s) \left[ \bm p_i^{gl} \beta_i^{s+} -  \bm p_i^{gu} \beta_i^{s-}  \right]  - \omega_i^{s} \right. & \notag \\
& \qquad \left. - \bm p_i^d \alpha_i^{s} \right\} - \sum_{(i,j) \in \mathcal E} \left\{ Mx_{ij}\xi_{ij}^{s} \left[ \delta_{ij}^{s+} + \delta_{ij}^{s-} \right] \right.  & \notag  \\
& \qquad  +  \left( \bm \theta_{ij} (1-x_{ij}\xi_{ij}^s) + \bm \theta^M x_{ij}\xi_{ij}^s\right) \left[ \eta_{ij}^{s+} + \eta_{ij}^{s-}\right] & \notag \\
& \qquad \left. + \,\bm t_{ij} (1 - x_{ij}{\xi}_{ij}^{s}) \left[ \gamma_{ij}^{s+} + \gamma_{ij}^{s-} \right] \right\}, & \label{eq:sd_n} \\
& \text{Eq. \eqref{eq:x}, \eqref{eq:kcl} -- \eqref{eq:loadshed_1}, and \eqref{eq:pij_d} -- \eqref{eq:nn_2} } \quad \forall s \in \mathcal S. & \notag 
\end{flalign}
The nonlinear terms in the formulation $\mathcal F_2$ are binary-continuous products $y_i\beta_i^{s+}$, $y_i\beta_i^{s-}$, $x_{ij} \delta_{ij}^{s+}$, $x_{ij} \delta_{ij}^{s-}$, $x_{ij} \gamma_{ij}^{s+}$, and $x_{ij} \gamma_{ij}^{s-}$; Mccormick relaxation is exact on these terms. {\color{blue} Finding suitable upper bounds on the continuous variables remains an open question.} Let $\mathcal F_3$ represent the resulting MILP obtained after applying Mccormick relaxation. Then, one can apply an L-shaped algorithm to decompose and solve $\mathcal F_3$.

\section{Alternate Formulation without McCormick relaxations}
An $N$-$k$ attack, $a \in \mathcal A^{k}$ is defined as $ \mathcal N^a \bigcup \mathcal E^a$ such that $|\mathcal N^a| + |\mathcal E^a| = k$. Similarly a scenario $s \in \mathcal S$, is defined as $\mathcal N^s \bigcup \mathcal E^s$. Let $\mathcal N(s,a) = \mathcal N^a \bigcap \mathcal N^s$ and $\mathcal E(s,a) = \mathcal E^a \bigcap \mathcal E^s$. Given an $N$-$k$ attack $a \in \mathcal A^k$ and a scenario $s \in \mathcal S$, the inner minimization problem can be formulated as follows: 
\begin{flalign*}
& \eta(s,a) = \min \, \sum_{i \in {\mathcal N}} \bm p^d_i \ell_i^s + (z-1) \sum_{i\in \mathcal N} \bm p^d_i &  \\
\text{ subject to:} && \notag \\
(\alpha_i^s)\quad & p_i^{gs} - (1-\ell_i^s)\bm p_i^d = \sum_{(i,j) \in \mathcal E \bigcup \mathcal E^r} p_{ij}^s \quad \forall i\in \mathcal N, &  \\
(\beta_i^{s+}, \beta_i^{s-})\quad & z \bm  p^{gl}_i \leqslant p^{gs}_i \leqslant z \bm  p^{gu}_i \quad \forall i \notin \mathcal N(s,a), &\\
(\kappa_i^{s+}, \kappa_i^{s-})\quad & z - |p^{gs}_i| \geqslant 1 \quad \forall i \in \mathcal N(s,a), & \\
(\gamma_{ij}^{s+}, \gamma_{ij}^{s-})\quad & z \bm t_{ij} - |p_{ij}^s| \geqslant 0 \quad \forall (i,j) \notin \mathcal E(s,a), & \\
(\delta_{ij}^{s+}, \delta_{ij}^{s-})\quad & z - |p_{ij}^s| \geqslant 1 \quad \forall (i,j) \in \mathcal E(s,a), & \\
(\phi_{ij}^s) \quad & p_{ij}^s + \bm b_{ij} (\theta^s_i - \theta^s_j) = 0  \quad \forall (i,j) \notin \mathcal E(s,a), & \\
(\omega_i^s) \quad &\ell_i^s \leqslant 1 \quad \forall i \in \mathcal N, &  \\
&\ell_i^s \geqslant 0 \quad \forall i \in \mathcal N. & 
\end{flalign*}
Given the primal for an attack $a \in \mathcal A^k$ and scenario $s \in \mathcal S$, an equivalent dual program is given as follows:
\begin{flalign*}
 & \Delta(s,a) = \max \, \sum_{i \in \mathcal N} \left( \kappa_i^{s+} + \kappa_i^{s-} - \omega_i^s - \bm p_i^d \alpha_i\right) & \notag \\
& \qquad\qquad\qquad + \sum_{(i,j) \in \mathcal E} \left(\delta_{ij}^{s+} + \delta_{ij}^{s-}\right) & \\
\text{subject to:} && \notag \\
(p_{ij}^s) \quad & \alpha_i^s - \alpha_j^s + \phi_{ij}^s + \gamma_{ij}^{s-} - \gamma_{ij}^{s+} +  \delta_{ij}^{s-} - \delta_{ij}^{s+} = 0 &\notag \\
& \hspace{25ex} \quad\forall (i,j) \in \mathcal E & \\
(p_i^{gs}) \quad & -\alpha_i^s + \beta_i^{s+} - \beta_i^{s-} + \kappa_i^{s+} - \kappa_i^{s-} = 0 \quad \forall i \in \mathcal N, & \\
(\theta_i^s) \quad & \sum_{(i,j) \in \mathcal E \bigcup \mathcal E^r} b_{ij} \phi_{ij}^s = 0 \quad \forall i \in \mathcal N, & \\
(\ell_i^s) \quad & -\bm p_i^d \alpha_i^s - \omega_i^s \leqslant \bm p_i^d \quad \forall i \in \mathcal N, & \\
(z) \quad & \sum_{(i,j) \in \mathcal E} \left( \delta_{ij}^{s+} + \delta_{ij}^{s-} + \bm t_{ij} ( \gamma_{ij}^{s+} + \gamma_{ij}^{s-} ) \right) + & \notag \\
 &\sum_{i \in \mathcal N} \left(\kappa_i^{s+} + \kappa_i^{s-} + \bm p_i^{gu} \beta_i^{s+} + \bm p_i^{gl} \beta_i^{s-} \right) \leqslant \sum_{i \in N} \bm p_i^d, & \\
 (\lambda_{ij}^{s+}, \lambda_{ij}^{s-}) \quad & |\phi_{ij}^s| \leqslant \bm M (1-x_{ij}) \quad \forall (i,j) \in \mathcal E, & \\
 (\varrho_{ij}^s) \quad & \bm t_{ij} (\gamma_{ij}^{s+} + \gamma_{ij}^{s-}) \leqslant (1 - x_{ij}) \sum_{i \in N} \bm p_i^d \quad \forall (i,j) \in \mathcal E, & \\
 (\mu_{ij}^s) \quad & \delta_{ij}^{s+} + \delta_{ij}^{s-} \leqslant (1 - x_{ij}) \sum_{i \in N} \bm p_i^d \quad \forall (i,j) \in \mathcal E, & \\
  (\psi_{i}^s) \quad & \bm p_i^{gu} \beta_{i}^{s+} + \bm p_i^{gl} \beta_{i}^{s-} \leqslant (1 - x_{ij}) \sum_{i \in N} \bm p_i^d \quad \forall i \in \mathcal N, & \\
 (\nu_{i}^s) \quad & \kappa_{i}^{s+} + \kappa_{i}^{s-} \leqslant (1 - x_{ij}) \sum_{i \in N} \bm p_i^d \quad \forall i \in \mathcal N, & \\
 & \beta_i^{s+}, \beta_i^{s-}, \kappa_i^{s+}, \kappa_i^{s-}, \omega_i^s \geqslant 0 \quad \forall i \in \mathcal N, & \\
& \gamma_{ij}^{s+}, \gamma_{ij}^{s-}, \delta_{ij}^{s+}, \delta_{ij}^{s-} \geqslant 0 \quad \forall (i,j) \in \mathcal E. & 
\end{flalign*}

\section{Solution Approach} \label{sec:saa}
The approach we present is a combination of sampling, decomposition, and parallel computing. This approach is refered to as the Sample Average Approximation for solving the SNKP. Suppose that the total number of components that can be interdicted in a given transmission network is $N$, and the probability of a successful interdiction on each component is independent of the other components in the system. Then we have $2^N = |\mathcal S|$ realization of uncertainty. This number of large scenarios makes direct use of the formulation $\mathcal F_3$ computationally intractable. Hence, we shall resort to a \textit{sample average} approach which has been shown to be effective in solving such stochastic programs (see \cite{}) with large number of scenarios. In the sample average approach, instead of maximizing the true expected load shed in the system from an $N$-$k$ attack, $$ f = \sum_{s\in \mathcal S} \bm{Pr}_s \left(\sum_{i \in \mathcal N} \bm p_i^d \ell_i^s \right),$$ we maximize a sample average approximation of $f$, given by $$ f_{\mathcal T} = \sum_{s\in \mathcal T} |\mathcal T|^{-1} \left(\sum_{i \in \mathcal N} \bm p_i^d \ell_i^s \right).$$


